Stability of Gradient Learning Dynamics in Continuous Games: Vector Action Spaces

Towards characterizing the optimization landscape of games, this paper analyzes the stability of gradient-based dynamics near fixed points of two-player continuous games. We introduce the quadratic numerical range as a method to characterize the spectrum of game dynamics and prove the robustness of equilibria to variations in learning rates. By decomposing the game Jacobian into symmetric and skew-symmetric components, we assess the contribution of a vector field's potential and rotational components to the stability of differential Nash equilibria. Our results show that in zero-sum games, all Nash are stable and robust; in potential games, all stable points are Nash. For general-sum games, we provide a sufficient condition for instability. We conclude with a numerical example in which learning with timescale separation results in faster convergence.

==> figs/qnr-toy2.tex <==

\begin{figure}[t]
\input{figs/qnr_toy}
\caption{
\emph{
%An  example of 
A stable
equilibrium that is not Nash.}
The spectrum of $\J$, $\J_{11}$, and $\J_{22}$ in Example~\ref{ex:qnum-toy} are 
contained
in the numerical range (convex dashed region) and quadratic numerical range (non-convex region) of $J$.
%
The eigenvalues of $J$ are in the left plane, hence the fixed point is stable under gradient play~\eqref{eq:gradientplay}.
However, the first player's $J_{11}$ is indefinite, hence the fixed point is not a Nash equilibrium.
%
%The eigenvalues of $\J_{11}$ and $\J_{22}$ are real.
%The quadratic numerical range 
%gives tight bounds on the spectrum of two-player games.
}
\label{fig:qnum-toy}
\end{figure}

==> figs/qnr_toy.tex <==
\centering
\begin{tikzpicture}
\begin{axis}[
width=.38\textwidth,
height=.34\textwidth,
thick,
axis on top,
%axis equal image,
axis x line=none,
axis y line = none,
ylabel={\small $\imag(\lambda)$},
xlabel={},
%xtick={-1,0,1},ytick={-1,0,1},
xtick=\empty,ytick=\empty,
xlabel style={below left},
ylabel style={below left},
clip=false]
%UNCOMMENT THIS IN THE FINAL VERSION
\addplot graphics
[xmin=-1.5,xmax=1,ymin=-1.5,ymax=1.5]
{figs/qnr.pdf};
%

%\draw [<-] (axis cs:-0.2,0.2) -- (axis cs:.5,.4) node [right ] {$\NR(\J)$}; 
\draw [<-] (axis cs:-0.5,-0.3) -- (axis cs:-.8,-.8) node [left  ] {$\QNR(\J)$}; 
\draw [-stealth] (axis cs:0,-1.3) -- (axis cs:0,1.3);
\draw (axis cs:.4, 1.1) node [right] {$\spec(J)$};
\draw (axis cs:.4, .68) node [right] {$\spec(J_{11})$};
\draw (axis cs:.4, .27) node [right] {$\spec(J_{22})$};
\draw [-stealth] (axis cs:0,0) -- (axis cs:1.5,0) node [below left] {\small $\real(\lambda)$};
\draw (axis cs:-1.5,0) -- (axis cs:-1.2,0);
\end{axis}
\end{tikzpicture}
